Induced gravitational waves -- beyond linear cosmological perturbation theory

This thesis focuses on gravitational waves (GWs) that arise beyond linear order in cosmological perturbation theory. In recent years, scalar-induced GWs have attracted significant attention because they may serve as the observational signature of primordial black holes (PBHs) formed in the early universe. The formation of PBHs requires large density perturbations, which can naturally emerge in some models of inflation. When these large density fluctuations couple, they act as a source for scalar-induced GWs at second order. In this work, we extend the existing formalism by including linear tensor fluctuations as an additional source term. This gives rise to two new classes of second-order GWs: those sourced by scalar-tensor couplings (scalar-tensor induced GWs) and those quadratic in tensor modes (tensor-tensor induced GWs). We find that the scalar-tensor contribution becomes significant if first-order tensor modes are enhanced, whilst the tensor-tensor contribution remains subdominant. Moreover, we demonstrate that the spectrum of scalar-tensor induced GWs exhibits an unphysical enhancement in the UV limit when the primordial scalar power spectrum is insufficiently peaked. To investigate whether this can be resolved, we study third-order induced GWs and their correlation with primordial GWs. We find that this new contribution suppresses the overall signal but does not cancel the unphysical enhancement. Possible explanations for this behaviour are discussed and left for future work. Finally, we explore the effect of primordial scalar non-Gaussianity on the spectrum of scalar-tensor induced GWs, building on previous results showing its impact on scalar-induced GWs.

==> macros.tex <==
% Abréviations maths

\newcommand\ph{\ensuremath{\varphi}}
\newcommand\eps{\ensuremath{\varepsilon}}

\newcommand{\cc}{\text{c.c.}}
\newcommand{\cst}{\mathrm{cst}}
\newcommand{\sgn}{\mathrm{sgn}}

%
\def\be{\begin{equation}}
\def\ee{\end{equation}}
%
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
%
\def\lb{\left(}
\def\rb{\right)}
\def\lbs{\left[}
\def\rbs{\right]}
\def\lbc{\left\{}
\def\rbc{\right\}}
%
\def\p{\partial}
\def\n{\nabla}
\def\dkk{\p_k\p^k}
\def\sh{{\sigma}}
\def\L{\pounds}
%\def\S{{\textgoth{S}}}
%\def\R2{{\textgoth{R}}}
%\def\S{{{\cal{S}}_2}}
\def\R{{{\cal{R}}}}
%\def\R1{{{\cal{R}}_1}}
\def\Va{{V_\alpha}}
\def\Q{{\cal{Q}}}
\def\ka{\kappa}
\def\eps{{\epsilon}}
\def\dr{{\delta\rho}}

\def\Ld{\pounds}
\def\T{\mathcal{T}}
\def\Hh{\mathcal{H}}
\def\M{\mathcal{M}}
\def\wt{\widetilde}
\def\ul{\underline}


%\newcommand\define{\overset{\text{déf.}}{=}}
\newcommand\define{\equiv}
\newcommand{\coordequal}{\overset{*}{=}}
\newcommand\alg[1]{\overline{#1}}
%\newcommand\vect[1]{\overrightarrow{#1}}
\newcommand\vect[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\boldsymbol{#1}}
\newcommand\cplx[1]{\underline{#1}}
\newcommand\ex[1]{\mathrm{e}^{#1}}
\renewcommand\i{\ensuremath{\mathrm{i}}}
\renewcommand\j{\ensuremath{\mathrm{j}}}
\renewcommand\Re{\ensuremath{\mathrm{Re}}}
\renewcommand\Im{\ensuremath{\mathrm{Im}}}
\newcommand{\Arg}{\ensuremath{\mathrm{Arg}}}
\newcommand\suite[3]{\ensuremath{(#1)_{#2\in{#3}}}}
\newcommand\transpose[1]{#1^{\rm T}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand\colonne[2]{\begin{pmatrix} #1 \\ #2 \end{pmatrix}}
\newcommand\gcolonne[2]{\begin{pmatrix} #1 \\[1mm] #2 \end{pmatrix}}
\newcommand\Ker{\mathrm{Ker}}

\def\X{{\cal{X}}}
\def\Xv{{{\cal{X}}_{v}}}
\def\XB{{{\cal{X}}_{B}}}
\def\Xpi{{{\cal{X}}_{\Pi}}}
\def\XNL{{{\cal{X}}_{\text{NL}}}}


\newcommand\e[1]{_{\text{#1}}}
\newcommand\h[1]{^{\text{#1}}}
\newcommand\U[1]{\:\mathrm{#1}}
\newcommand{\micro}{\hbox{\textmu}}

\newcommand{\rm}{\mathrm{d}}
\newcommand{\Dd}{\mathrm{D}}
\newcommand{\pd}[3][]{\frac{\partial^{#1} #2}{\partial {#3}^{#1}}}
\newcommand{\ddf}[3][]{\frac{\dd^{#1} #2}{\dd {#3}^{#1}}}
\newcommand{\Ddf}[3][]{\frac{\Dd^{#1} #2}{\dd {#3}^{#1}}}

\newcommand{\grad}{\vect{\nabla}}

%\renewcommand\lim[2]{\underset{ #1 \rightarrow #2 }{ \mathrm{lim} } \,}
\newcommand\tendvers[2]{\underset{#1 \rightarrow #2}{\longrightarrow}}

\newcommand{\delimiters}[4][]{
\ifthenelse{ \equal{#1}{1} }{  #2 #3 #4  }
					{ \ifthenelse{\equal{#1}{2}}{ \big#2 #3 \big#4 }
						{ \ifthenelse{\equal{#1}{3}}{ \Big#2 #3 \Big#4 }
							{ \ifthenelse{\equal{#1}{4}}{ \bigg#2 #3 \bigg#4 }
								{ \ifthenelse{\equal{#1}{5}}{ \Bigg#2 #3 \Bigg#4 }
									{ \left#2 #3 \right#4 }
								}
							}
						}
					}
													}

\newcommand{\pa}[2][]{\delimiters[#1]{(}{#2}{)}}
\newcommand{\pac}[2][]{\delimiters[#1]{[}{#2}{]}}
\newcommand{\paac}[2][]{\delimiters[#1]{\{}{#2}{\}}}
\newcommand{\abs}[2][]{\delimiters[#1]{|}{#2}{|}}
\newcommand{\ev}[2][]{\delimiters[#1]{\langle}{#2}{\rangle}}
\newcommand{\evaluate}[2][]{\delimiters[#1]{.}{#2}{|}}
\newcommand{\mean}[2][]{\delimiters[#1]{\langle}{#2}{\rangle}}
\newcommand{\ket}[2][]{\delimiters[#1]{|}{#2}{\rangle}}
\newcommand{\bra}[2][]{\delimiters[#1]{\langle}{#2}{|}}



\newcommand{\lp}[1]{\color{red}{(lp: #1)}\color{black}}
\newcommand{\hubble}{\mathcal{H}}
\newcommand{\invplanck}{M_{Pl}^{-2}}
\newcommand{\conf}{^{\prime}}
\newcommand{\cs}{c_s^2}
\newcommand{\conv}{\mathbf{k}-\mathbf{p}}
\newcommand{\bareta}{\overline{\eta}}
\newcommand{\barx}{\overline{x}}
\newcommand{\tildeeta}{\tilde{\eta}}
\newcommand{\tildey}{\tilde{y}}
%\newcommand{\eps}{\epsilon}
\newcommand{\timeder}{\partial _{\eta}}
\newcommand{\timederbar}{\partial _{\overline{\eta}}}
\newcommand{\avant}{ \left ( \frac{3+3w}{5+3w} \right ) }
\newcommand{\munu}{_{\mu \nu}}
\newcommand{\back}{^{(0)}}
\newcommand{\second}{^{(2)}}
\newcommand{\third}{^{(3)}}
\newcommand{\four}{(2\pi)^{\frac{3}{2}}}

\newcommand{\source}{\mathrm{s}}
\newcommand{\obs}{\mathrm{o}}
\newcommand{\PF}[1]{\textcolor{red}{#1}}
\newcommand{\varDA}{\sigma_{D\e{A}}^2}

\newcommand{\tidal}{\mathcal{R}}
\newcommand{\jacobi}{\mathcal{D}}
\newcommand{\wronski}{\mathcal{W}}
\newcommand{\amplification}{\mathcal{A}}
\newcommand{\deformation}{\mathcal{S}}
\newcommand{\Ricfoc}{\mathscr{R}}
\newcommand{\Weylfoc}{\mathscr{W}}

\newcommand{\Lie}{\mathcal{L}}
\newcommand{\wl}{\mathscr{L}}

\newcommand{\Hc}{\mathcal{H}}

\newcommand{\nul}[1]{%\hat{#1}
#1}

\newcommand{\zero}{\mat{0}}
\newcommand{\identity}{\mat{1}}


\DeclareRobustCommand{\rchi}{{\mathpalette\irchi\relax}}
\newcommand{\irchi}[2]{\raisebox{\depth}{$#1\chi$}}
\def\<{\langle}
\def\>{\rangle}


\newenvironment{system}
{ \left\{ \begin{aligned} }
{ \end{aligned} \right. }

\newenvironment{remark}
{

\medskip

\noindent
\hspace{0.05\linewidth}
\vline
\hspace{0.01\linewidth}
\begin{minipage}{0.93\linewidth}
}
{
\end{minipage}

\medskip

}

% Box
\newlength{\boxtitlelength}
\newlength{\halfrulelength}
\newcommand{\boxtitle}[1]{\footnotesize\bf{\:#1\:}}
\newenvironment{abox}[1]
{
\setlength{\halfrulelength}{0.5\linewidth}
\settowidth{\boxtitlelength}{\boxtitle{#1}}
\addtolength{\halfrulelength}{-0.5\boxtitlelength}
\noindent\rule[-1mm+1pt]{1pt}{2mm}\rule[1mm]{\halfrulelength}{1pt}{\boxtitle{#1}}\rule[1mm]{\halfrulelength}{1pt}\rule[-1mm+1pt]{1pt}{2mm}\\}
{\\ \rule[1mm]{1pt}{2mm}\noindent\rule[1mm]{\linewidth-2pt}{1pt}\rule[1mm]{1pt}{2mm}}

% Create a command for sections hidden in the text
\newcommand{\hiddensection}[1]{
\refstepcounter{section}
\phantomsection
\addcontentsline{toc}{section}{\protect\numberline{\thesection}#1}
\markright{\thesection \: #1}
}

% Colors

\definecolor{blue4}{RGB}{0,0,143}
\definecolor{red4}{RGB}{143,0,0}
\definecolor{orange}{RGB}{255,128,0}
\definecolor{darkcyan}{RGB}{0,128,128}
\definecolor{olive}{RGB}{0,128,0}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{cyan2}{RGB}{0,255,255}
\definecolor{fushia}{RGB}{255,0,255}
\definecolor{mygray}{gray}{0.5}
\definecolor{lightgray}{gray}{0.85}

% Journals

\newcommand{\apj}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\apjl}{ApJL}
\newcommand{\aap}{A{\&}A}
\newcommand{\aaps}{A{\&}AS}
\newcommand{\mnras}{MNRAS}
\newcommand{\aj}{AJ}
\newcommand{\araa}{ARAA}
\newcommand{\pasp}{PASP}
\newcommand{\pasj}{PASJ}
\newcommand{\jcap}{JCAP}
\newcommand{\na}{New Astronomy}
\newcommand{\physrep}{Phys. Rep.}
\newcommand{\prd}{Phys. Rev. D}
\newcommand{\azh}{Astron. Zh.}
\newcommand{\nat}{Nature}
\newcommand{\nar}{New Astronomy Reviews}

